Scaling Binarized Neural Networks on Reconfigurable Logic

Binarized neural networks (BNNs) are gaining interest in the deep learning community due to their significantly lower computational and memory cost. They are particularly well suited to reconfigurable logic devices, which contain an abundance of fine-grained compute resources and can result in smaller, lower power implementations, or conversely in higher classification rates. Towards this end, the Finn framework was recently proposed for building fast and flexible field programmable gate array (FPGA) accelerators for BNNs. Finn utilized a novel set of optimizations that enable efficient mapping of BNNs to hardware and implemented fully connected, non-padded convolutional and pooling layers, with per-layer compute resources being tailored to user-provided throughput requirements. However, FINN was not evaluated on larger topologies due to the size of the chosen FPGA, and exhibited decreased accuracy due to lack of padding. In this paper, we improve upon Finn to show how padding can be employed on BNNs while still maintaining a 1-bit datapath and high accuracy. Based on this technique, we demonstrate numerous experiments to illustrate flexibility and scalability of the approach. In particular, we show that a large BNN requiring 1.2 billion operations per frame running on an ADM-PCIE-8K5 platform can classify images at 12 kFPS with 671 us latency while drawing less than 41 W board power and classifying CIFAR-10 images at 88.7% accuracy. Our implementation of this network achieves 14.8 trillion operations per second. We believe this is the fastest classification rate reported to date on this benchmark at this level of accuracy.

==> content/backup/2-bkg.tex <==
\section{Background}
A great deal of prior work on mapping neural networks to hardware exist for \glspl{FPGA}, GPUs and ASICs to help increase inference rate or improve energy efficiency.
We refer the reader to the work by Misra and Saha~\cite{surveyannhw} for a comprehensive survey whereby we distinguish four basic architecture:
1) a \textit{single processing engine}, usually in the form of a \textit{systolic array}, which processes each layer sequentially~\cite{ovtcharov2015accelerating,zhang2015optimizing,chen2016eyeriss,YodaNN};
2) a \textit{streaming architecture}~\cite{venieris2016fpgaconvnet,alemdar2016ternary}, consisting of one processing engine per network layer;
3) a \textit{vector processor}~\cite{farabet2009cnp} with instructions specific to accelerating the primitives operations of convolutions; and
4) a \textit{neurosynaptic processor}~\cite{esser2016convolutional}, which implements many digital neurons and their interconnecting weights.
Complementary to these basic architectural choices, numerous compression techniques are being investigated~\cite{han2015deep, iandola2016squeezenet, iandola2015firecaffe}
One of several possible dimensions is reducing precision \cite{ResiliencyUnderQuantization} with the extreme manifestation being \glspl{BNN} whereby either input activations, synapse weights or output activations or a combination thereof are binarized.
%We consider three aspects of binarization for neural network layers: binary input activations, binary synapse weights and binary output activations. If all three components are binary, we refer to this as 
\textit{Full binarization} is leveraged by Kim~and~Smaragdis~\cite{bitwiseneuralnet}.
The seminal XNOR-Net work by Rastegari~et~al.~\cite{xnornet} applies convolutional \glspl{BNN} on the ImageNet dataset with topologies inspired by AlexNet, ResNet and GoogLeNet, reporting top-1 accuracies of up to 51.2\% for full binarization and 65.5\% for \textit{partial binarization}.
DoReFa-Net by Zhou~et~al.~\cite{dorefa} explores reduced precision during the forward pass as well as the backward pass, and note that this opens interesting possibilities for training neural networks on \glspl{FPGA}. Their results include configurations with partial and full binarization on the SVHN and ImageNet datasets, including best-case ImageNet top-1 accuracies of 43\% for full and 53\%  for partial binarization.
Finally, the work by Courbariaux~et~al.~\cite{binarynet} describes how to train fully-connected and convolutional networks with full binarization and batch normalization layers, reporting competitive accuracy on the MNIST, SVHN and CIFAR-10 datasets. The authors are not aware of any prior publication that investigates mapping of fully binarized neural networks onto FPGAs, while we are aware that there are a few pending submissions to upcoming conferences. Amongst those, we believe that our architecture is conceptually different with its full dataflow nature and to the best of our knowledge outperforms every other implementation.



==> content/backup/3b-architecture-opts.tex <==
\textbf{BNN-specific Operator Optimizations.}
\label{sec:Optimizations}
\glspl{BNN} have several properties that enable a more efficient mapping to \glspl{FPGA} without affecting the network accuracy, which we describe in the following subsections.
We assume that the methodology described in \cite{binarynet} is used for training all \glspl{BNN} in this paper, where all \gls{BNN} layers have the following properties (unless otherwise stated). Firstly, we are using 1-bit values for all input activations, weights and output activations (full binarization), where an unset bit represents -1 and a set bit represents +1. Secondly, batch normalization prior to the activation function. finally, we are using the following activation function: \\
    $\mathrm{Sign}(x) = 
\{+1 \text{~if~} x \geq 0, -1 \text{~if~} x < 0\}$
Further detail is provided below.

\textbf{Popcount for Accumulation.}
\label{sec:Popcount}
The regular and value-constrained nature of \gls{BNN} computations enable computing binary dot products with fewer hardware resources.
The practical consequence for hardware implementations of a sum operations is that the summation of a binary dot product can be implemented by a \emph{popcount} operation that counts the number of set bits instead of accumulation with signed arithmetic.
%Our experiments with Vivado HLS indicate that popcount-accumulate requires approximately half the number of LUT and FF resources to implement compared to signed-accumulate.
%For instance, with a target $F_{\mathrm{clk}}=200$~MHz, a 128-bit popcount-accumulate requires 376 LUTs and 29 FFs, while a 128-bit bipolar-accumulate requires 759 LUTs and 84 FFs.
% Vivado 2015.4
% Target Fclk: 200 MHz
% Target device: xc7z045ffg900-2
% using 16-bit acc
% Source: snippets/popcount-vs-bipolar.cpp

%               LUT     FF      clk (ns)
% popcount-32   88      0       4.20
% bipolar-32    184     18      3.25
% popcount-64   185     17      4.20
% bipolar-64    376     37      4.20
% popcount-128  376     29      4.20
% bipolar-128   759     84      4.20
% popcount-256  759     53      4.20
% bipolar-256   1526    162     4.20

\textbf{Batchnorm-activation as Threshold.}
\label{sec:BatchnormToThres}

All \gls{BNN} layers use batch normalization \cite{batchnorm} on convolutional or fully connected layer outputs, then apply the sign function to determine the output activation. In \cite{finn} we show how the same output can be computed via thresholding.
Using these techniques, we can compute the output activation using an unsigned comparison and avoid computing the batch normalized value altogether during inference.
$\tau_k^+$ itself is fixed for a trained network and can be computed from the batchnorm parameters at compile time.
%Synthesis reports from Vivado HLS for 16-bit dot product output values indicate that regular batchnorm-and-sign activation requires 2 DSPs, 55 FFs and 40 LUTs, whereas the threshold activation we describe here only requires 6 LUTs.

\textbf{Boolean OR for Max-pooling.}
\label{sec:BinPooling}
The networks described in \cite{binarynet} perform pooling prior to activations, i.e. pooling is performed on non-binarized numbers, which are then batch normalized and fed into the activation function, however as we show in \cite{finn}, pooling can be equally performed after activation, once binarized, in which case it can be effectively implemented with the Boolean OR-operator.
%We show that the same layer outputs can be derived by max pooling \emph{after} the activations without having to re-train the network.
%Let $a_1, a_2, \ldots a_Y$ be the positive dot product outputs that will be processed by max-pooling.
%The output would be computed as $a^b = (\mathrm{Max}(a_1, a_2, \ldots a_Y) > \tau^+)$.
%Due to the distributivity of $\mathrm{Max}$, the output will be $\mathnormal{true}$ if \emph{any} of $a_1, a_2, \ldots a_S$ are greater than $\tau^+$.
%Therefore, the same result can be computed as $a^b = (a_1 > \tau^+) \vee (a_2 > \tau^+) \ldots \vee (a_Y > \tau^+)$.
%As the threshold comparisons are already computed for the activations, max-pooling can be effectively implemented with the Boolean OR-operator.
Similar principles apply for min-pooling (as Boolean AND) and average-pooling (as Boolean majority function) as well.

%\subsubsection{Hardcoding weights into LUT equations}
%\TODO{describe the potential benefits from hardcoding: no explicit weight memories, LUTs for XNOR disappear, logic synthesis engine can apply additional optimizations. mention experimental results and limitations on current devices.}


==> content/backup/3c-architecture-components.tex <==
\subsection{FINN Design Flow and Hardware Library}
\label{sec:BuildingBlocks}

%\begin{figure}
%    \centering
%    \includegraphics[height=3.5cm]{images/bnn-workflow-horizontal.pdf}
%    \caption{Generating an FPGA accelerator from a trained \gls{BNN}.}
%    \label{fig:workflow}
%\end{figure}

Figure \ref{fig:workflow-summary} illustrates the design flow for converting a trained BNN into an FPGA accelerator.
%This flow assumes the \gls{BNN} has been trained in the Theano framework \cite{theano} using the methodology described by Courbariaux et al. \cite{binarynet} which produces a trained network in the form of a NumPy archive (.npz).
The user supplies a \gls{FPS} target alongside a Theano-trained \gls{BNN} to the \OurScheme{} synthesizer.
The synthesizer first determines the folding parameters (Section \ref{sec:Folding}) to meet the \gls{FPS} target and applies the optimizations from Section \ref{sec:Optimizations}, then produces a synthesizable C++ description of a heterogeneous streaming architecture.
The architecture is composed of building blocks from the \OurScheme{} hardware library described in the following subsections.

%\begin{itemize}
%    \item A trained \gls{BNN} in the form of a NumPy archive (.npz) from Theano, which contains the network topology and all parameters associated with layers.
%    \item A set of parameters that describe how each layer will be folded to create a hardware architecture that matches the throughput requirements. The relationship between the folding parameters and classification throughput in described in Section TODO.
%\end{itemize}
%With these inputs, the following steps are executed:
%\begin{enumerate}
%    \item A Python script generates a .cpp file that instantiates the HLS components which correspond to the \gls{BNN} layers. This script is also responsible for converting the \gls{BNN} parameters to the format expected by the accelerator, including converting biases and batch normalization parameters to threshold values as described in Section \ref{sec:BatchnormToThres}. It also generates a set of files to initialize the accelerator memories with the \gls{BNN} parameters.
%    \item Vivado HLS takes in the generated .cpp file and the library of templated, parametrizable streaming component implementations, generates a pipelined design according to the provided FPGA model and frequency constraints, and generates a Vivado IP core ready for synthesis.
%    \item A tcl script sets up a Vivado project using the generated IP core and any platform-specific constraints, performs synthesis, place and route, and generates a bitfile with the desired hardware architecture.
%\end{enumerate}

%All the building blocks described in this section are implemented in Vivado HLS as templated C++ functions, each of which correspond to one type of a neural network layer.
%Each component uses streaming interfaces for input and output, and contains a single loop (a common iteration space) pipelined with a target \gls{II} of 1.
%The top-level \gls{BNN} compute function itself consists of a series of function calls and stream variable declarations to instantiate the necessary layers and the data streams between them.
%The \texttt{dataflow} pragma is used on the top-level to overlap communication and computation between layers, thereby minimizing the completion latency.

\subsubsection{The Matrix--Vector--Threshold Unit}
\label{sec:MVTU}
\begin{figure}
    \centering
    \includegraphics[height=3cm]{images/mvu-overview.pdf}
    \caption{Overview of the MVTU.}
    \label{fig:MVUOverview}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[height=3.2cm]{images/pe-datapath.pdf}
    \caption{MVTU PE datapath. \textbf{Bold} indicates bitwidth.}
    \label{fig:PEDatapath}
\end{figure}

The \gls{MVU} forms the computational core for our accelerator designs.
The vast majority of compute operations in a \gls{BNN} can be expressed as matrix--vector operations followed by thresholding.
For instance, the pre-activation output $\mathbf{a_N}$ of the fully connected neural network layer at index $N$ is given by matrix-vector product $\mathbf{a_N} = \mathbf{A} \cdot \mathbf{a^b_{N-1}}$ where $\mathbf{A}$ is the synaptic weight matrix and $\mathbf{a^b_{N-1}}$ are the activations from the previous layer.
The post-activation output can then be computed by $\mathbf{a^b_N} = \mathbf{a^N} > \mathbf{\tau^+_N}$, where the thresholds $\mathbf{\tau^+_N}$ are determined as described in Section \ref{sec:BatchnormToThres}.
Convolutions can also be implemented as matrix--vector products, as will be described in Section \ref{sec:ConvImpl}.
As such, the \gls{MVU} implements fully-connected layers as a standalone component, and is also used as part of the convolutional layers.

The overall organization of the \gls{MVU} is shown in Figure \ref{fig:MVUOverview}.
Internally, the \gls{MVU} consists of an input and output buffer, and an array of \glspl{PE} each with a number of SIMD lanes.
The number of \glspl{PE} ($P$) and SIMD lanes ($S$) are configurable to control the throughput as discussed in Section \ref{sec:FoldingMatrixVector}.
The synapse weight matrix to be used is kept in \gls{OCM} distributed between \glspl{PE}, and the input images stream through the \gls{MVU} as each one is multiplied with the matrix.
Each \gls{PE} receives exactly the same control signals and input vector data, but multiply-accumulates the input with a different part of the matrix.
In terms of the taxonomy described in \cite{chen2016eyeriss}, this architecture is both \emph{weight stationary} (since each weight remains local to the \gls{PE}) and \emph{output stationary} (since each popcount computation remains local to the \gls{PE}).

Figure \ref{fig:PEDatapath} shows the datapath of an \gls{MVU} \gls{PE}.
It computes the dot product between the input vector and a row of the synaptic weight matrix and compares the result to a threshold, produceing a single-bit output.
The dot product computation itself is a multiply-accumulate operation between the two bit vectors and implemented with an XNOR gate. Following this, the number of set bits in the result is counted (see Section \ref{sec:Popcount}) and added to the accumulator register.
Once the entire dot product is accumulated, it is thresholded.
The accumulator, adder and threshold memory are $T$-bits wide, which can be scaled down to $T=1+\mathrm{log}_{2}(Y)$ for additional resource savings.

Finally, it is worth pointing out that the \gls{MVU} architectural template can also support partial binarization for non-binarized outputs and inputs.
Removing the thresolding stage provides non-binarized outputs, while using regular multiply-add instead of XNOR-popcount can handle non-binarized inputs
These features are used in the first and last layers of networks that process non-binary input images or do not output a one-hot classification vector.

\subsubsection{Convolution: The Sliding Window Unit}
\label{sec:ConvImpl}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/conv-lowering.pdf}
%     \caption{Lowering convolutions to matrix--matrix multiplication.}
%     \label{fig:ConvLowering}
% \end{figure}

Convolutions can be \emph{lowered} to matrix-matrix multiplications \cite{chellapilla2006high}, which is the approach followed in this work.
%Figure \ref{fig:ConvLowering} illustrates how 
The weights from the convolution filters are packed into a \emph{filter matrix}, while a sliding window is moved across input images to form an \emph{image matrix}.
These matrices are then multiplied to generate the output images.

\begin{figure}
	\centering
	\begin{subfigure}[t]{0.8\linewidth}
	  \centering
	  \includegraphics[width=\linewidth]{images/conv-interleaving.pdf}
	  \caption{\small Lowering with interleaved channels.}
	  \label{fig:ConvInterleaving}
	\end{subfigure}

	\begin{subfigure}[t]{0.8\linewidth}
		\centering
		\includegraphics[width=\linewidth]{images/conv-mems-interleaved.pdf}
		\caption{\small SWU operation.}
		\label{fig:SWUImpl}
	\end{subfigure}

	\caption{Convolution using interleaved channels.}
\end{figure}

The convolutional layer consists of a \gls{SWU}, which generates the image matrix from incoming feature maps, and a \gls{MVU} that actually computes the matrix--matrix product using a different column vector from the image matrix each time.
In order to better cater for the SIMD parallelism of the \gls{MVU} and minimize buffering requirements, we \emph{interleave} the feature maps such that each pixel contains all the \gls{IFM} channel data for that position, as illustrated in Figure \ref{fig:ConvInterleaving}.
Since the dot product to compute a \gls{OFM} pixel includes all \glspl{IFM} pixels at a certain sliding window location, those \gls{IFM} pixels can be processed in any order owing to the commutative property of addition.
Note that interleaving the filter matrix has no additional cost since it is done offline, and interleaving the input image can be done on-the-fly in the FPGA.
Storing the pixels in this fashion allows us to implement the \gls{SWU} with a single wide \gls{OCM} instead of multiple narrow \glspl{OCM}, and also enables the output of the \gls{MVU} to be directly fed to the next layer without any transposition.
As illustrated in Figure \ref{fig:SWUImpl}, the incoming \gls{IFM} data is simply stored at sequential addresses in a buffer, then the memory locations corresponding to each sliding window are read out to produce the image matrix.

%A straightforward solution would be to dedicate a single \gls{OCM} to each channel's image data, storing the pixels in row-major order and generating the sliding window by accessing individual memory locations, as illustrated in Figure TODO.
%However, implementing the \gls{SWU} in this manner presents two problems.
%The first problem is regarding \gls{OCM} resources: there may be hundreds of channels in a single layer of a \gls{CNN}, which would rapidly consume the available \gls{OCM} on the \gls{FPGA}.
%The second problem is regarding data layout when feeding a convolutional layer's output into the next convolutional layer's input: the \gls{MVU} produces its output one column at a time, so feeding this column-major output to the input of a row-major \gls{SWU} would require an expensive transpose operation.
%\TODO{we need to explain what we're doing to avoid ping pong buffers- thereby minimizing buffer reuqirements- we're laying out the matrix such that can produce and consume between layers in "roughly" the same order", reference eyeriss again}

Although not required by any of the networks described in this work, the \gls{SWU} also pads the images if necessary.
One interesting observation is that with the bipolar number representation used in this work, there is no number corresponding to zero.
Therefore, in order to maintain a true binary datapath for activations, images must be padded with our representation or either a 1 or a -1.
Future work will look into what impact this has on the accuracy of trained networks, but early experiments suggest that there is very little difference in accuracy, with respect to \cite{binarynet}.

\subsubsection{The Pooling Unit}
The \gls{PU} implements max-pooling as described in Section \ref{sec:BinPooling}.
To implement $k \times k$ max-pooling on a $D_H \times D_W$ binary image of $C$ channels, the \gls{PU} contains $C \cdot k$ line buffers of $D_W$ bits each.
As with the rest of our component library, the \gls{PU} operates in a streaming fashion.
The input image is gradually streamed into the line buffers.
When at least $k$ rows of the image have arrived, each $k$ consecutive bits of the line buffer are OR'ed together to produce horizontal subsampling for each channel.
These are then OR'ed together with the other line buffers to produce vertical subsampling, the results are streamed out, and the oldest line buffers are refilled with the next row of pixels.
%Currently our \gls{PU} only supports max-pooling with OR-reduction, though other Boolean reduction functions such as majority-bit for average pooling (Section \ref{sec:BinPooling}) would be straightforward to implement.


==> content/backup/3d-folding.tex <==
\subsection{Folding}
\label{sec:Folding}
In terms of the \gls{MVU} description given in Section \ref{sec:MVTU}, each \gls{PE} corresponds to a \emph{hardware neuron}, while each SIMD lane acts as a \emph{hardware synapse}.
If we were to dimension each \gls{MVU} in a network with a number of hardware neurons and synapses equal to the number of neurons and synapses in a \gls{BNN} layer, this would result in a fully parallel neural network that could classify images at the clock rate.
However, the amount of hardware resources on an \gls{FPGA} is limited, and it is necessary to time-multiplex (or \emph{fold}) the \gls{BNN} onto fewer hardware synapses and neurons.
We now describe how the folding is performed subject to user constraints.

The work by Venieris et al. \cite{venieris2016fpgaconvnet} describes a method for folding neural networks expressed as streaming dataflow graphs, with focus on formalizing the folding and design space exploration.
In this work, we consider a simpler variant that only controls the folding of matrix--vector products to achieve a given \gls{FPS} requirement set by the user, and focus on \emph{how} the folding is implemented in terms of the workload mapping.
As almost all computations in \glspl{BNN} are expressed as matrix--vector multiplications, implementing folding for matrix--vector multiplication already enables a great degree of control over the system throughput.
Folding directly affects the resource and power consumption of the final system as well, which we explore in Section \ref{sec:results}.

\subsubsection{Folding Matrix--Vector Products}
\label{sec:FoldingMatrixVector}
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/mvu-folding.pdf}
    \caption{Neuron and synapse folding for \gls{MVU}.}
    \label{fig:MVUMapping}
\end{figure}

Folding matrix--vector products is achieved by controlling two parameters of the \gls{MVU}: $P$ the number of \glspl{PE}, and $S$ the number of SIMD lanes per \gls{PE}.
These determine how the matrix is partitioned between the \glspl{PE}.
A $P$-high, $S$-wide tile of the matrix is processed at a time, with each row in the tile mapped to a different PE, and each column to a different SIMD lane.
For a $X \times Y$ matrix, we refer to $F^n = X / P$ as the \emph{neuron fold} and $F^s = Y / S$ as the \emph{synapse fold}.
The \emph{total fold} $F$ is then obtained as $F = F^n \cdot F^s$, which is also the number of cycles required to complete one matrix--vector multiply.
Note that $F^n$ and $F^s$ should be integers to avoid padding the weight matrix.
As an example, Figure \ref{fig:MVUMapping} shows how a $6\times4$  weight matrix is partitioned between three \glspl{PE} with two SIMD lanes each.
Here, each matrix-vector multiply will take $F^n \cdot F^s = (6 / 3) \cdot (4 / 2) = 4$ cycles.

The same principle applies for convolutional layers, but these always have an inherent amount of folding due to our current matrix--matrix product as multiple matrix--vector products implementation.
For convolutional layers, the total fold is $F = F^m \cdot F^n \cdot F^s$, where 
$F^m$ is a network-dependent constant due to multiple matrix-vector products, and is equal to the number of output pixels from the convolution.

\subsubsection{Determining $F^n$ and $F^s$}
Avoiding the \dblquotes{one-size-fits-all} inefficiencies requires tailoring each \gls{MVU}'s compute resources to layer requirements.
The guiding principle here is \emph{rate-balancing} the heterogeneous streaming architecture: the slowest layer (with $II_{\mathrm{max}}$) will determine the overall throughput, so each layer should use a roughly equal number of cycles to process one image.
As this is a streaming system, the classification throughput $\mathrm{FPS}$ will be approximately $\frac{F_{\mathrm{clk}}}{II_{\mathrm{max}}}$, where $F_{\mathrm{clk}}$ is the clock frequency.
For a fully-connected layer, the total fold $F$ is equal to the \gls{II}.
Therefore, balancing a fully-connected \gls{BNN} can be achieved by using $F^n$ and $F^s$ such that $F^n \cdot F^s = \frac{F_{\mathrm{clk}}}{\mathrm{FPS}}$ for each layer.
Depending on the \gls{BNN} and the \gls{FPS} requirements, the number of memory channels or sliding window generation may constitute bottlenecks.
For such cases, we match the throughput of all other layers to the bottleneck in order not to waste resources.


==> content/backup/3e-padding.tex <==
\subsection{Padding With Non-zero Values}
\label{sec:padding}

BinaryNet~\cite{binarynet} goes to significant lengths to ensure that the networks they describe can be implemented with an \textit{almost} fully binarized datapath.
The authors train networks with weights constrained to 2 values, the activation functions they use are also constrained to only 2 values, both with -1/1 represented as 0/1 respectively.
The only places a non-binarized datapath is required is when the popcount/thresholds are computed and when padding is used in convolutional layers.
Padding is used to better detect features that are close to the edge of images, and involves adding extra pixels around an image which are set to zero.
In order to implement convolutions on the \gls{MVU} one would likely have to either:
1) insert zeros into the input vectors where it is appropriate; or
2) introduce valid signals along with each value to selectively include it into the calculation or not.
The issue with both methods 1) and 2), is that an extra bit would be required for each value on the datapath.
While adding an extra bit to the datapath would not usually incur a significant hardware cost,
for binarized networks, this means \textit{doubling} the bitwidth of the datapath and as such likely to incur a significant handware cost.

In this work, a fully binarized datapath datapath is preferred.
As such, we use the method described in 1) but the zeros we insert correspond to -1 values, rather than 0 values.
The implications of this padding type on the accuracy of the resultant networks is discussed briefly in Section~\ref{sec:results}.



==> fig/brameff.tex <==
\begin{tikzpicture}
\begin{axis}[
			xlabel={\% relative to allocated},
			xbar stacked, bar width=6pt,
			enlarge y limits={abs=0.3cm},
			width=7cm, height=3.2cm,
			y=0.5cm,
            area legend,
			legend style={font=\scriptsize},
			legend pos={outer north east},
			legend columns=1,
            legend image code/.code={\draw[#1] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);},
			ytick=data,
			xmin=0,
			xmax=100,
			symbolic y coords={cnnf14,cnnf12,cnns1},
            yticklabels={\cnns{1},\cnnf{1}{2},\cnnf{1}{4}},
			]
			
%\addplot+[ybar] coordinates {					
%(\cnf{1}{4}, 5184)
%(\cnf{1}{2}, 13896)
%(\cnns{1}, 65304)
%};					
%\addlegendentry{allocated}					
					
%\addplot+[ybar] coordinates {					
%(\cnf{1}{4}, 858)
%(\cnf{1}{2}, 3428)
%(\cnns{1}, 13695)
%};					
%\addlegendentry{params}										
%
%\addplot+[ybar] coordinates {					
%(\cnf{1}{4}, 113)
%(\cnf{1}{2}, 198)
%(\cnns{1}, 368)
%};					
%\addlegendentry{buffers}

\addplot coordinates {					
(21.0,cnns1)
(24.7,cnnf12)
(16.55,cnnf14)
};					
\addlegendentry{params}										

\addplot coordinates {					
(4.506335573,cnns1)	
(11.14285501,cnnf12)
(14.94163231,cnnf14)
};					
\addlegendentry{buffers}

\addplot coordinates {					
(74.5,cnns1)	
(64.15714499,cnnf12)
(68.5084,cnnf14)
};					
\addlegendentry{unused}

\end{axis}

\end{tikzpicture}


==> fig/cifar10-acc-cost.tex <==
\begin{tikzpicture}
\begin{semilogxaxis}[
	width=0.5\columnwidth,
	%height=4cm,
    xlabel={Computational Cost},
    ylabel={Error (\%)},
    log basis x=10,
    %xticklabel=\pgfmathparse{2^\tick}\pgfmathprintnumber{\pgfmathresult},
    %xticklabels={0.125, 1, 8, 64, 512, 4096, 16384, 32768},
    %log ticks with fixed point,
    %xmin=0.125, xmax=32768,
    %ymin=1, ymax=100000,
    legend pos={north east},
    legend style={
    	%at={(0.5,1.03)},
    	%anchor=south,
    	font=\scriptsize
    },
    legend columns=1
]
   
\addplot
    table [x=rel_cost_f32, y=test_err_f32, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-cost-f32};
\addplot
    table [x=rel_cost_16bit, y=test_err_16bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-cost-i16};
\addplot
    table [x=rel_cost_8bit, y=test_err_8bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-cost-i8};
\addplot
    table [x=rel_cost_4bit, y=test_err_4bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-cost-i4};
\addplot
    table [x=rel_cost_2bit, y=test_err_2bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-cost-i2};
\addplot
    table [x=rel_cost_bin, y=test_err_bin, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-cost-bin};

\legend{FP, Int16, Int8, Int4, Int2, Bin.}
\end{semilogxaxis}
\end{tikzpicture}
%
\begin{tikzpicture}
\begin{semilogxaxis}[
	width=0.5\columnwidth,
	%height=4cm,
    xlabel={Memory size (bits)},
    ylabel={Error (\%)},
    log basis x=10,
    %xticklabel=\pgfmathparse{2^\tick}\pgfmathprintnumber{\pgfmathresult},
    %xticklabels={0.125, 1, 8, 64, 512, 4096, 16384, 32768},
    %log ticks with fixed point,
    %xmin=0.125, xmax=32768,
    %ymin=1, ymax=100000,
    legend pos={north east},
    legend style={
    	%at={(0.5,1.03)},
    	%anchor=south,
    	font=\scriptsize
    },
    legend columns=1
]
   
\addplot
    table [x=mem_f32, y=test_err_f32, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-f32};
\addplot
    table [x=mem_16bit, y=test_err_16bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-i16};
\addplot
    table [x=mem_8bit, y=test_err_8bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-i8};
\addplot
    table [x=mem_4bit, y=test_err_4bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-i4};
\addplot
    table [x=mem_2bit, y=test_err_2bit, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-i2};
\addplot
    table [x=mem_bin, y=test_err_bin, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-bin};
\addplot+[mark=none]
    table [x=v7690t_mem, y=vert, col sep=comma] {csv/Cifar10-acc-cost.csv};
    \label{cifar10-acc-mem-dev};

\legend{FP, Int16, Int8, Int4, Int2, Bin., Dev.}
\end{semilogxaxis}
\end{tikzpicture}

%\node [draw,fill=white] at (rel axis cs: 0.81,0.2) {\shortstack[l]{
%\scriptsize \ref{16-bit precision-ZU19EG} 16-bit ops - FPGA \\
%%\ref{8-bit precision-ZU19EG} 8-bit ops - FPGA\\
%\scriptsize \ref{1-bit precision-ZU19EG} 1-bit ops - FPGA\\
%\scriptsize \ref{Floating point precision-K40} 16-bit ops - GPU\\
%\scriptsize \ref{1-bit precision-K40} 1-bit ops - GPU
%}};


==> fig/roofline-7v3.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[
	width=\linewidth,
	height=4.5cm,
    xlabel={Ops:Byte},
    ylabel={GOps/s},
    log basis x=2,
    % YU: I commented this out because it was making compilation
    % fail with a "dimension too large" error.
    %xticklabel=\pgfmathparse{2^\tick}\pgfmathprintnumber{\pgfmathresult},
    xticklabels={0.125, 2, 32, 512, 8192, 131072},
    %log ticks with fixed point,
    xmin=0.125, xmax=524288,
    ymin=1, ymax=100000,
    legend pos={north west},
    legend style={
    	%at={(0.5,1.03)},
    	%anchor=south,
    	font=\scriptsize
    },
    legend columns=1
]
   
\addplot[
    dashed, thick, 
    color=blue,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ADM_PCIe_7V3-FP, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{FP precision-7v3};
\addplot[
    dotted, thick,
    color=black,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ADM_PCIe_7V3-8b, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{8-bit precision-7v3};
\addplot[
    dashdotted, thick,
    color=red,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ADM_PCIe_7V3-4b, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{4-bit precision-7v3}; 
%\addplot[
%    loosely dotted, thick,
%    color=purple,
%    mark=none,
%    ]
%    table [x=OperationalIntensity, y=ADM_PCIe_7V3-2b, col sep=comma] {fig/csv/Roofline-7v3.csv};
%    \label{2-bit precision-7v3};     
\addplot[
    densely dashdotted, thick,
    color=gray,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ADM_PCIe_7V3-1b, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{1-bit precision-7v3}; 
\addplot [color=brown, thick, name path global=quarter] coordinates {
		(25340,1)
		(25340,100000)};
    \label{quarter};
\addplot [color=brown, thick, mark=*] coordinates {
		(25340,937)};
\addplot [color=gray, thick, name path global=half] coordinates {
		(100213,1)
		(100213,100000)};
    \label{half};
\addplot [color=gray, thick, mark=*] coordinates {
		(100213,3711)};
\addplot [color=green, thick, name path global=full] coordinates {
		(398558,1)
		(398558,100000)};
    \label{full};
\addplot [color=green, thick, mark=*] coordinates {
		(398558,7838)};
\addplot [color=purple, thick, name path global=half_nopad] coordinates {
		(38461,1)
		(38461,100000)};
    \label{half_nopad};
\addplot [color=purple, thick, mark=*] coordinates {
		(38461,1613)};
%\legend{FP ops, 8-bit ops, 4-bit ops, 2-bit ops, 1-bit ops}
\end{loglogaxis}



\node [draw,fill=white] at (rel axis cs: 0.3,0.8) {\shortstack[l]{
\ref*{FP precision-7v3} FP32 \\
\ref*{8-bit precision-7v3} 8-bit \\
\ref*{4-bit precision-7v3} 4-bit \\
%\ref*{2-bit precision-7v3} 2-bit \\
\ref*{1-bit precision-7v3} 1-bit}};

% Second "Legend" node
\node [draw,fill=white] at (rel axis cs: 0.7,0.2) {\shortstack[l]{
%\ref*{LeNEt} LeNEt \\
%\ref*{AlexNet complete} AlexNet complete \\
\ref*{full} Full \\
\ref*{half} Half \\
\ref*{quarter} Quarter \\
\ref*{half_nopad} Half w/o pad 
}};

\end{tikzpicture}


==> fig/roofline-ku115.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[
	height=4cm,
	width=0.85\linewidth,
    xlabel={Ops:Byte},
    ylabel={GOps/s},
    log basis x=2,
    % YU: I commented this out because it was making compilation
    % fail with a "dimension too large" error.
    %xticklabel=\pgfmathparse{2^\tick}\pgfmathprintnumber{\pgfmathresult},
    xticklabels={0.125, 2, 32, 512, 8192, 131072},
    %log ticks with fixed point,
    xmin=0.125, xmax=524288,
    ymin=1, ymax=100000,
    legend pos={north west},
    legend style={
    	%at={(0.5,1.03)},
    	%anchor=south,
    	font=\scriptsize
    },
    legend columns=1
]
   
\addplot[
    dashed, thick, 
    color=blue,
    mark=none,
    ]
    table [x=OperationalIntensity, y=KU115-FP, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{FP precision-7v3};
\addplot[
    dotted, thick,
    color=black,
    mark=none,
    ]
    table [x=OperationalIntensity, y=KU115-8b, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{8-bit precision-7v3};
\addplot[
    dashdotted, thick,
    color=red,
    mark=none,
    ]
    table [x=OperationalIntensity, y=KU115-4b, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{4-bit precision-7v3}; 
%\addplot[
%    loosely dotted, thick,
%    color=purple,
%    mark=none,
%    ]
%    table [x=OperationalIntensity, y=KU115-2b, col sep=comma] {fig/csv/Roofline-7v3.csv};
%    \label{2-bit precision-7v3};     
\addplot[
    densely dashdotted, thick,
    color=gray,
    mark=none,
    ]
    table [x=OperationalIntensity, y=KU115-1b, col sep=comma] {fig/csv/Roofline-7v3.csv};
    \label{1-bit precision-7v3}; 
\addplot [color=brown, thick, name path global=quarter] coordinates {
		(25340,1)
		(25340,100000)};
    \label{quarter};
\addplot [color=brown, thick, mark=*] coordinates {
		(25340,937)};
\addplot [color=gray, thick, name path global=half] coordinates {
		(100213,1)
		(100213,100000)};
    \label{half};
\addplot [color=gray, thick, mark=*] coordinates {
		(100213,3711)};
\addplot [color=green, thick, name path global=full] coordinates {
		(398558,1)
		(398558,100000)};
    \label{full};
\addplot [color=green, thick, mark=*] coordinates {
		(398558,14814)};
%\addplot [color=purple, thick, name path global=half_nopad] coordinates {
%		(38461,1)
%		(38461,100000)};
%    \label{half_nopad};
%\addplot [color=purple, thick, mark=*] coordinates {
%		(38461,1613)};
%\legend{FP ops, 8-bit ops, 4-bit ops, 2-bit ops, 1-bit ops}
\end{loglogaxis}



\node [draw,fill=white] at (rel axis cs: 0.3,0.75) {\shortstack[l]{
\ref*{FP precision-7v3} FP32 \\
\ref*{8-bit precision-7v3} 8-bit \\
\ref*{4-bit precision-7v3} 4-bit \\
%\ref*{2-bit precision-7v3} 2-bit \\
\ref*{1-bit precision-7v3} 1-bit}};

% Second "Legend" node
\node [draw,fill=white] at (rel axis cs: 0.7,0.28) {\shortstack[l]{
%\ref*{LeNEt} LeNEt \\
%\ref*{AlexNet complete} AlexNet complete \\
\ref*{full} cnn(1) \\
\ref*{half} cnn(1/2) \\
\ref*{quarter} cnn(1/4)
%\ref*{half_nopad} cnn$_{_{NoPad}}$(1/2)
%\ref*{half_nopad} cnn\textsubscript{NoPad}(1/2)
}};

\end{tikzpicture}


==> images/roofline_ku115.tex <==
\begin{tikzpicture}
\begin{loglogaxis}[
	width=\columnwidth,
	height=4cm,
    xlabel={Ops:Byte},
    ylabel={GOps/s},
    log basis x=2,
    % YU: I commented this out because it was making compilation
    % fail with a "dimension too large" error.
    %xticklabel=\pgfmathparse{2^\tick}\pgfmathprintnumber{\pgfmathresult},
    xticklabels={0.125, 1, 8, 64, 512, 4096, 16384, 32768},
    %log ticks with fixed point,
    xmin=0.125, xmax=32768,
    ymin=1, ymax=100000,
    legend pos={north west},
    legend style={
    	%at={(0.5,1.03)},
    	%anchor=south,
    	font=\scriptsize
    },
    legend columns=1
]

%\addplot[
%    solid, thick,
%    color=brown,
%    mark=none,
%    ]
%    table [x=OperationalIntensity, y=K40, col sep=comma] {csv-graph/Roofline-updated.csv};
%    \label{Floating point precision-K40}; 
%    
%\addplot[
%    solid, thick,
%    color=violet,
%    mark=none,
%    ]
%    table [x=OperationalIntensity, y=K40-1b, col sep=comma] {csv-graph/Roofline-updated.csv};
%    \label{1-bit precision-K40}; 
%    
\addplot[
    dashed, thick, 
    color=blue,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ZU19EG-HP, col sep=comma] {csv-graph/Roofline-updated.csv};
    \label{16-bit precision-ZU19EG};
\addplot[
    dotted, thick,
    color=black,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ZU19EG-QP, col sep=comma] {csv-graph/Roofline-updated.csv};
    \label{8-bit precision-ZU19EG};
\addplot[
    dashdotted, thick,
    name path global=1bit,
    color=red,
    mark=none,
    ]
    table [x=OperationalIntensity, y=ZU19EG-1b, col sep=comma] {csv-graph/Roofline-updated.csv};
    \label{1-bit precision-ZU19EG}; 
\addplot [color=violet,thick, name path global=DoreFanet] coordinates {
		(9602,1)
		(9602,100000)};
    \label{AlexNet};
\addplot [color=violet, thick, mark=*] coordinates {
		(9602,40000)};   

\addplot [color=green,thick, name path global=AlexNet8BitOffChip] coordinates {
		(23.28,1)
		(23.28,100000)};
    \label{AlexNet8BitOffChip};
\addplot [color=green, thick, mark=*] coordinates {
		(23.28,111.74)};

\draw (5, 3) node[rotate=90]{\tiny 8-bit};
\draw (5.5, 2.7) node[rotate=90]{\tiny all off-chip};


\draw (13.5, 3) node[rotate=90]{\tiny 1-bit};
\draw (14.0, 2.7) node[rotate=90]{\tiny all on-chip};
		
\legend{16-bit ops, 8-bit ops, 1-bit ops}
\end{loglogaxis}

%\node [draw,fill=white] at (rel axis cs: 0.81,0.2) {\shortstack[l]{
%\scriptsize \ref{16-bit precision-ZU19EG} 16-bit ops - FPGA \\
%%\ref{8-bit precision-ZU19EG} 8-bit ops - FPGA\\
%\scriptsize \ref{1-bit precision-ZU19EG} 1-bit ops - FPGA\\
%\scriptsize \ref{Floating point precision-K40} 16-bit ops - GPU\\
%\scriptsize \ref{1-bit precision-K40} 1-bit ops - GPU
%}};
\end{tikzpicture}

==> tables/accuracy-cifar10.tex <==
%\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cccccccc}
\toprule
              & Binary    & Int2      & Int4      & Int8      & Int16     & Float     & &\\
Scale Factor  & Err. (\%) & Err. (\%) & Err. (\%) & Err. (\%) & Err. (\%) & Err. (\%) & \# Params  & Ops/frame\\
\midrule
0.25          & 20.94     & 16.05     & 14.81     & 14.29     & 14.15     & 15.44     & 879,914    & 78,494,720\\
0.5           & 14.84     & 0.97      & 0.97      & 0.97      & 0.97      & 12.14     & 3,510,858  & 310,343,680\\
1.0           & 11.67     & 0.91      & 0.91      & 0.91      & 0.91      & 10.76     & 14,025,866 & 1,234,104,320\\
\bottomrule
\end{tabular}
%TODO: Add the real fixed values from AWS results.
%}


==> tables/accuracy-fc-mnist.tex <==
%\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cccccccc}
\toprule
              & Binary    & Int2      & Int4      & Int8      & Int16     & Float     & &\\
Neurons/layer & Err. (\%) & Err. (\%) & Err. (\%) & Err. (\%) & Err. (\%) & Err. (\%) & \# Params & Ops/frame\\
\midrule
%1 & 78.99 & 66.97 & 66.97 & 66.97 & 66.97 & 66.97 & 809 & 1,592\\
%2 & 79.14 & 56.86 & 56.86 & 56.86 & 56.86 & 1,612 & 3,192\\
%4 & 79.68 & 53.71 & 53.71 & 53.71 & 53.71 & 3,230 & 6,416\\
%8 & 63.31 & 39.74 & 39.74 & 39.74 & 39.74 & 6,514 & 12,960\\
%16 & 49.87 & 23.34 & 23.34 & 23.34 & 23.34 & 13,274 & 26,432\\
%32 & 22.12 & 8.35 & 8.35 & 8.35 & 8.35 & 27,562 & 54,912\\
64 & 10.89  & 4.99 & 4.99 & 4.99 & 4.99 & 4.99 & 59,210 & 118,016\\
128 & 6.58  & 2.70 & 2.70 & 2.70 & 2.70 & 2.70 & 134,794 & 268,800\\
256 & 4.17  & 1.78 & 1.78 & 1.78 & 1.78 & 1.78 & 335,114 & 668,672\\
512 & 2.31  & 1.25 & 1.25 & 1.25 & 1.25 & 1.25 & 932,362 & 1,861,632\\
1024 & 1.60 & 1.13 & 1.13 & 1.13 & 1.13 & 1.13 & 2,913,290 & 5,820,416\\
2048 & 1.32 & 0.97 & 0.97 & 0.97 & 0.97 & 0.97 & 10,020,874 & 20,029,440\\
4096 & 1.17 & 0.91 & 0.91 & 0.91 & 0.91 & 0.91 & 36,818,954 & 73,613,312\\
\bottomrule
\end{tabular}
%TODO: Add the real fixed values from AWS results.
%}


==> tables/cifar10.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c | c c }
\toprule
$Layer \#$ & $Layer Type$ & $Type_{in}$ & $W_{in}$ & $H_{in}$ & $Ch_{in}$ & $Type_{out}$ & $W_{out}$ & $H_{out}$ & $Ch_{out}$  & $Kernel$ & $PoolDim$ & $P$ & $S$\\
\midrule
1  & Convolutional    & 8-bit  & 32 & 32  & 3   & Binary & 30 & 30  & 64  & 3 & - & 64  & 3 \\
2  & Convolutional    & Binary & 30 & 30  & 64  & Binary & 28 & 28  & 64  & 3 & - & 64  & 64 \\
3  & Max pooling      & Binary & 28 & 28  & 64  & Binary & 14 & 14  & 64  & - & 2 & -   & - \\
4  & Convolutional    & Binary & 14 & 14  & 64  & Binary & 12 & 12  & 128 & 3 & - & 32  & 64 \\
5  & Convolutional    & Binary & 12 & 12  & 128 & Binary & 10 & 10  & 128 & 3 & - & 32  & 64 \\
6  & Max pooling      & Binary & 10 & 10  & 128 & Binary & 5  & 5   & 128 & - & 2 & -   & - \\
7  & Convolutional    & Binary & 5  & 5   & 128 & Binary & 3  & 3   & 256 & 3 & - & 8   & 64 \\
8  & Convolutional    & Binary & 3  & 3   & 256 & Binary & 1  & 1   & 256 & 3 & - & 2   & 64 \\
9  & Fully Connected  & Binary & -  & 256 & -   & Binary & -  & 512 & -   & - & - & 1   & 16 \\
10 & Fully Connected  & Binary & -  & 512 & -   & Binary & -  & 512 & -   & - & - & 1   & 32 \\
11 & Fully Connected* & Binary & -  & 512 & -   & 16-bit & -  & 10  & -   & - & - & 4   & 1 \\
\midrule
1  & Convolutional    & 8-bit  & 32 & 32  & 3   & Binary & 32 & 32  & 32  & 3 & - & -   & - \\
2  & Convolutional    & Binary & 32 & 32  & 32  & Binary & 32 & 32  & 32  & 3 & - & -   & -  \\
3  & Max pooling      & Binary & 32 & 32  & 32  & Binary & 16 & 16  & 32  & - & 2 & -   & - \\
4  & Convolutional    & Binary & 16 & 16  & 32  & Binary & 16 & 16  & 64  & 3 & - & -   & -  \\
5  & Convolutional    & Binary & 16 & 16  & 64  & Binary & 16 & 16  & 64  & 3 & - & -   & -  \\
6  & Max pooling      & Binary & 16 & 16  & 64  & Binary & 8  & 8   & 64  & - & 2 & -   & - \\
7  & Convolutional    & Binary & 8  & 8   & 64  & Binary & 8  & 8   & 128 & 3 & - & -   & -  \\
8  & Convolutional    & Binary & 8  & 8   & 128 & Binary & 8  & 8   & 128 & 3 & - & -   & -  \\
9  & Max pooling      & Binary & 8  & 8   & 128 & Binary & 4  & 4   & 128 & - & 2 & -   & - \\
10 & Fully Connected  & Binary & -  & 2048& -   & Binary & -  & 256 & -   & - & - & -   & -  \\
11 & Fully Connected  & Binary & -  & 256 & -   & Binary & -  & 256 & -   & - & - & -   & -  \\
12 & Fully Connected* & Binary & -  & 256 & -   & 16-bit & -  & 10  & -   & - & - & -   & - \\
\midrule
1  & Convolutional    & 8-bit  & 32 & 32  & 3   & Binary & 32 & 32  & 64  & 3 & - & -   & - \\
2  & Convolutional    & Binary & 32 & 32  & 64  & Binary & 32 & 32  & 64  & 3 & - & -   & -  \\
3  & Max pooling      & Binary & 32 & 32  & 64  & Binary & 16 & 16  & 64  & - & 2 & -   & - \\
4  & Convolutional    & Binary & 16 & 16  & 64  & Binary & 16 & 16  & 128 & 3 & - & -   & -  \\
5  & Convolutional    & Binary & 16 & 16  & 128 & Binary & 16 & 16  & 128 & 3 & - & -   & -  \\
6  & Max pooling      & Binary & 16 & 16  & 128 & Binary & 8  & 8   & 128 & - & 2 & -   & - \\
7  & Convolutional    & Binary & 8  & 8   & 128 & Binary & 8  & 8   & 256 & 3 & - & -   & -  \\
8  & Convolutional    & Binary & 8  & 8   & 256 & Binary & 8  & 8   & 256 & 3 & - & -   & -  \\
9  & Max pooling      & Binary & 8  & 8   & 256 & Binary & 4  & 4   & 256 & - & 2 & -   & - \\
10 & Fully Connected  & Binary & -  & 4096& -   & Binary & -  & 512 & -   & - & - & -   & -  \\
11 & Fully Connected  & Binary & -  & 512 & -   & Binary & -  & 512 & -   & - & - & -   & -  \\
12 & Fully Connected* & Binary & -  & 512 & -   & 16-bit & -  & 10  & -   & - & - & -   & - \\
\midrule
1  & Convolutional    & 8-bit  & 32 & 32  & 3   & Binary & 32 & 32  & 128 & 3 & - & -   & - \\
2  & Convolutional    & Binary & 32 & 32  & 128 & Binary & 32 & 32  & 128 & 3 & - & -   & -  \\
3  & Max pooling      & Binary & 32 & 32  & 128 & Binary & 16 & 16  & 128 & - & 2 & -   & - \\
4  & Convolutional    & Binary & 16 & 16  & 128 & Binary & 16 & 16  & 256 & 3 & - & -   & -  \\
5  & Convolutional    & Binary & 16 & 16  & 256 & Binary & 16 & 16  & 256 & 3 & - & -   & -  \\
6  & Max pooling      & Binary & 16 & 16  & 256 & Binary & 8  & 8   & 256 & - & 2 & -   & - \\
7  & Convolutional    & Binary & 8  & 8   & 256 & Binary & 8  & 8   & 512 & 3 & - & -   & -  \\
8  & Convolutional    & Binary & 8  & 8   & 512 & Binary & 8  & 8   & 512 & 3 & - & -   & -  \\
9  & Max pooling      & Binary & 8  & 8   & 512 & Binary & 4  & 4   & 512 & - & 2 & -   & - \\
10 & Fully Connected  & Binary & -  & 8192& -   & Binary & -  & 1024& -   & - & - & -   & -  \\
11 & Fully Connected  & Binary & -  & 1024& -   & Binary & -  & 1024& -   & - & - & -   & -  \\
12 & Fully Connected* & Binary & -  & 1024& -   & 16-bit & -  & 10  & -   & - & - & -   & - \\
%\midrule
%1  & Convolutional    & 8-bit  & 32 & 32  & 3           & Binary & 32 & 32  & 128$\sigma$& 3 & - & -   & - \\
%2  & Convolutional    & Binary & 32 & 32  & 128$\sigma$ & Binary & 32 & 32  & 128$\sigma$& 3 & - & -   & -  \\
%3  & Max pooling      & Binary & 32 & 32  & 128$\sigma$ & Binary & 16 & 16  & 128$\sigma$& - & 2 & -   & - \\
%4  & Convolutional    & Binary & 16 & 16  & 128$\sigma$ & Binary & 16 & 16  & 256$\sigma$& 3 & - & -   & -  \\
%5  & Convolutional    & Binary & 16 & 16  & 256$\sigma$ & Binary & 16 & 16  & 256$\sigma$& 3 & - & -   & -  \\
%6  & Max pooling      & Binary & 16 & 16  & 256$\sigma$ & Binary & 8  & 8   & 256$\sigma$& - & 2 & -   & - \\
%7  & Convolutional    & Binary & 8  & 8   & 256$\sigma$ & Binary & 8  & 8   & 512$\sigma$& 3 & - & -   & -  \\
%8  & Convolutional    & Binary & 8  & 8   & 512$\sigma$ & Binary & 8  & 8   & 512$\sigma$& 3 & - & -   & -  \\
%9  & Max pooling      & Binary & 8  & 8   & 512$\sigma$ & Binary & 4  & 4   & 512$\sigma$& - & 2 & -   & - \\
%10 & Fully Connected  & Binary & -  & 8192$\sigma$& -   & Binary & -  & 1024$\sigma$& -   & - & - & -   & -  \\
%11 & Fully Connected  & Binary & -  & 1024$\sigma$& -   & Binary & -  & 1024$\sigma$& -   & - & - & -   & -  \\
%12 & Fully Connected* & Binary & -  & 1024$\sigma$& -   & 16-bit & -  & 10  & -   & - & - & -   & - \\
\midrule[.5pt]
\multicolumn{12}{l}{\textsuperscript{*}\footnotesize{Layer with no activation}}
\end{tabular}
}


==> tables/fcmnist.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c | c c }
\toprule
$Layer \#$ & $Layer Type$ & $Type_{in}$ & $W_{in}$ & $H_{in}$ & $Ch_{in}$ & $Type_{out}$ & $W_{out}$ & $H_{out}$ & $Ch_{out}$  & $Kernel$ & $PoolDim$ & $P$ & $S$\\
\midrule
1 & Fully Connected  & Binary & -  & 784 & -  & Binary & -  & 256  & -  & - & - & 256 & 64 \\
2 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 256  & -  & - & - & 64  & 64 \\
3 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 256  & -  & - & - & 64  & 64 \\
4 & Fully Connected  & Binary & -  & 256 & -  & Binary & -  & 10        & -  & - & - & 16  & 10 \\
\midrule
1 & Fully Connected  & Binary & -  & 784 & -  & Binary & -  & 512  & -  & - & - & 256 & 64 \\
2 & Fully Connected  & Binary & -  & 512 & -  & Binary & -  & 512  & -  & - & - & 128  & 64 \\
3 & Fully Connected  & Binary & -  & 512 & -  & Binary & -  & 512  & -  & - & - & 128  & 64 \\
4 & Fully Connected  & Binary & -  & 512 & -  & Binary & -  & 10        & -  & - & - & 16  & 10 \\
\midrule
1 & Fully Connected  & Binary & -  & 784        & -  & Binary & -  & 1024       & -  & - & - & 128 & 64 \\
2 & Fully Connected  & Binary & -  & 1024       & -  & Binary & -  & 1024       & -  & - & - & 128 & 64 \\
3 & Fully Connected  & Binary & -  & 1024       & -  & Binary & -  & 1024       & -  & - & - & 128 & 64 \\
4 & Fully Connected  & Binary & -  & 1024       & -  & Binary & -  & 10         & -  & - & - & 16  & 10 \\
%\midrule
%1 & Fully Connected  & Binary & -  & 784        & -  & Binary & -  & 1024$\sigma$ & -  & - & - & 128 & 64 \\
%2 & Fully Connected  & Binary & -  & 1024$\sigma$ & -  & Binary & -  & 1024$\sigma$ & -  & - & - & 128 & 64 \\
%3 & Fully Connected  & Binary & -  & 1024$\sigma$ & -  & Binary & -  & 1024$\sigma$ & -  & - & - & 128 & 64 \\
%4 & Fully Connected  & Binary & -  & 1024$\sigma$ & -  & Binary & -  & 10         & -  & - & - & 16  & 10 \\
\midrule[.5pt]
%\multicolumn{12}{l}{\textsuperscript{*}\footnotesize{The same network architecture has been implemented with several number of neurons (1024, 512, 256)}}\\
\multicolumn{12}{l}{\footnotesize{$Type_{in}$-$Type_{out}$: datatype of input/output feature map}}\\
\multicolumn{12}{l}{\footnotesize{$W_{in}$-$W_{out}$: width of input/output feature map}}\\
\multicolumn{12}{l}{\footnotesize{$H_{in}$-$H_{out}$: height of input/output feature map}}\\
\multicolumn{12}{l}{\footnotesize{$Ch_{in}$-$Ch_{out}$: input/output feature map channels}} \\
\multicolumn{12}{l}{\footnotesize{$P$-$S$: number of PEs and number of SIMD lanes per PE}}
%\multicolumn{12}{l}{\footnotesize{$\sigma$: A scale factor to explore different sized \glspl{MLP}}}
\end{tabular}
}


==> tables/networks.tex <==
\newcommand{\tss}[1]{\textsuperscript{#1}} % Some defines to make the tables easier to read.
\resizebox{\linewidth}{!}{
%\begin{tabularx}{\linewidth}{lrrrrrrrrrr}
\begin{tabular}{lrrrrrrrrrrr}
\toprule
Network         & \mlp{}        & \mlp{}       & \mlp{}       & \mlp{}      & \cnn{}       & \cnn{}       & \cnn{}     & \cnn{}       & \cnn{}       & \cnn{}     & \cnnnp{}     \\
%Network         & \mlp{}        & \mlp{}       & \mlp{}       & \mlp{}      & \cnn{}       & \cnn{}       & \cnn{}     & \cnn{}       & \cnn{}       & \cnn{}     & \cnnnp{}     \\
\midrule
$\sigma$        &$\rfrac{1}{16}$&$\rfrac{1}{8}$&$\rfrac{1}{4}$& $1$         &$\rfrac{1}{4}$&$\rfrac{1}{2}$& $1$        &$\rfrac{1}{4}$&$\rfrac{1}{2}$& $1$        &$\rfrac{1}{2}$\\
Dataset         & MNIST         & MNIST        & MNIST        & MNIST\tss{*}& CIFAR-10     & CIFAR-10     & CIFAR-10   & CIFAR-10     & CIFAR-10     & CIFAR-10   & CIFAR-10     \\
Pad Value       & -             & -            & -            & -           & 0            & 0            & 0          & -1           & -1           & -1         & -            \\
Ops/frame       & 669k          & 1,682k       & 5,820k       & 73,613k     & 78,495k      & 310,344k     & 1,234,104k & 78,495k      & 310,344k     & 1,234,104k & 118,970k     \\
Parameters      & 335k          & 932k         & 2,913k       & 36,819k     & 880k         & 3,509k       & 14,026k    & 880k         & 3,509k       & 14,026k    & 1,545k       \\
Test Err.(\%)   & 4.17          & 2.31         & 1.60         & 1.17        & 21.76        & 14.82        & 11.40      & 20.94        & 14.84        & 11.67      & 19.90        \\
%\midrule
%Alemdar~et~al.~\cite{alemdar2016ternary} & MNIST & Kintex-7 160T & 2 & 2.24 & 255.10 & 0.32 & - & 806.45 & - & \approxtilde{96.68} \\
%%Alemdar~et~al.~\cite{alemdar2016ternary}  & MNIST & Kintex-7 160T & 2 & 1.87 & 255.10 & 0.62 & - & 409.84 & - &\approxtilde{128.57} \\
%Alemdar~et~al.~\cite{alemdar2016ternary} & MNIST & Kintex-7 160T & 2 & 1.71 & 255.10 & 1.84 & - & 138.50 & - & \approxtilde{448.47} \\
%Alemdar~et~al.~\cite{alemdar2016ternary} & MNIST & Kintex-7 160T & 2 & 1.67 & 255.10 & 2.76 & - & 92.59 &  - & \approxtilde{864.03} \\
%Park and Sung~\cite{park2016fpga} & MNIST & ZC706 & 3 & - & 70 & 4.98 & - & 14.06 & - & \approxtilde{210} \\
%TrueNorth~\cite{esser2016convolutional} & CIFAR-10 & TrueNorth & 1 & 16.59 & 1.249 & 0.2044 & - & 6.11 & - & - \\
%TrueNorth~\cite{esser2016convolutional} & SVHN & TrueNorth & 1 & 3.34 & 2.526 & 0.2565 & - & 9.85 & - & - \\
%\midrule
%CaffePresso~\cite{caffepresso} & MNIST & Keystone-II & 16  & - & 5 & - & 14 & - & 0.357 & 44.82 \\
%CaffePresso~\cite{caffepresso} & CIFAR-10 & Keystone-II & 16  & - & 10 & - & 14 & - & 0.714 & 146.14 \\
%CaffePresso~\cite{caffepresso} & MNIST & Parallella & 32 & - & 0.64 & - & 5 & - & 0.129 & 5.78 \\
%CaffePresso~\cite{caffepresso} & CIFAR-10 & Parallella & 32  & - & 0.1 & - & 5 & - & 0.019 & 1.40 \\
%Ovtcharov~et~al.~\cite{ovtcharov2015accelerating} & CIFAR-10 & Stratix V D5 & 32 & \approxtilde{11-26} & 2.32 & - & 25 & - & 0.093 & - \\
\bottomrule
\multicolumn{12}{l}{\tss{*}\footnotesize{Non-binarized input images}}\\
\end{tabular}
%\end{tabularx}
}
\let\tss\undefined
%\vspace{\tabpad}


==> tables/op-cost.tex <==
%\resizebox{0.4\linewidth}{!}{
%\begin{tabularx}{\linewidth}{lrrrr}
\begin{tabular}{lrrrrrrrrr}
\toprule
Datatype & LUTs & LUTs & LUTs & DSPs  & DSPs  & DSPs  & $C_{avg}$       & $C_{rel}$\\
         & min  & max  & avg  & min   & max   & avg   & $\times 10^{-6}$&\\
\midrule
% Data from Gianluca's experiments.
Binary   & 2.16 & 4.25 & 2.90 & 0     & 0     & 0     & 9.56         & 1\\
Int2     & 5.57 & 9.95 & 7.03 & 0     & 0     & 0     & 23.17        & 2.42\\
Int4     & 13.81& 18.89& 15.60& 0     & 0     & 0     & 51.45        & 5.38\\
Int8     & 42.29& 44.78& 48.83& 0     & 0     & 0     & 147.7        & 15.45\\
Int16    & 10.99& 20.38& 15.03& 0.5   & 0.5   & 0.5   & 138.9        & 14.53\\
% Data from Michaela's spreadsheet.
Float32  & 356  & -    & -    & 4     & -     & -     & 587.0        & 61.41\\
\midrule
XC7VX690T& -    & 433,200 & - & -     & 3,600 & -     & -            & -\\
\bottomrule
\end{tabular}
%\end{tabularx}
%}


==> tables/workloads.tex <==
%\begin{tabularx}{\linewidth}{l|cccc}
\begin{tabular}{l|cccc}
\toprule
Topology & Params & Ops & Off-chip I/O & Op.Int.\\
 & (Mbits) & (M) & (B) &  (Ops/B) \\
\midrule
SFC & 0.3 & 0.6 & 112 & 5970 \\
LFC & 2.9 & 5.8 & 112 & 51968 \\
CNV & 1.5 & 112.5 & 3092 & 36400 \\
\midrule
Prototype & \multicolumn{4}{c}{Per-Layer Total Fold $(F)$} \\
\midrule
SFC-max & \multicolumn{4}{c}{13, 16, 16, 16} \\
LFC-max & \multicolumn{4}{c}{104, 128, 128, 128} \\
CNV-max & \multicolumn{4}{c}{8100, 7056, 5184, 7200, 5184, 4608, 8192, 8192, 1280} \\
\bottomrule
%\end{tabularx} 
\end{tabular} 

